INDIGO: Page Migration for Hardware Memory Disaggregation Across a Network

Hardware memory disaggregation (HMD) is an emerging technology that enables access to remote memory, thereby creating expansive memory pools and reducing memory underutilization in datacenters. However, a significant challenge arises when accessing remote memory over a network: increased contention that can lead to severe application performance degradation. To reduce the performance penalty of using remote memory, the operating system uses page migration to promote frequently accessed pages closer to the processor. However, previously proposed page migration mechanisms do not achieve the best performance in HMD systems because of obliviousness to variable page transfer costs that occur due to network contention. To address these limitations, we present INDIGO: a network-aware page migration framework that uses novel page telemetry and a learning-based approach for network adaptation. We implemented INDIGO in the Linux kernel and evaluated it with common cloud and HPC applications on a real disaggregated memory system prototype. Our evaluation shows that INDIGO offers up to 50-70% improvement in application performance compared to other state-of-the-art page migration policies and reduces network traffic up to 2x.

==> 0000-introduction.tex <==
\section{Introduction}
\label{s:introduction}

%The assumption of extreme network contention will be a factor when migrating remote memory doesn't seem like a plausible one, as it's likely to be local to a rack and attached to a switch with full bisection bandwidth.
%memory contention is realistic similar to common applications such as file transfer

%add figure showing runtime degradation of the applications for NUMA, NUMA with contention, HMD, HMD with contention

\noindent \textbf{Background.}
Hardware memory disaggregation (HMD) is an emerging technology that enables access to remote memory, thereby creating expansive memory pools and reducing memory underutilization in datacenters.
Previous work, using production datacenter traces, shows that HMD systems can increase memory utilization by 25\% and unlock massive cost savings~\cite{li2023pond,duraisamy2023towards}.
To enable remote memory access, HMD systems redirect memory accesses via dedicated memory interconnects, and employ state-of-the-art interconnect protocols such as CXL or OpenCAPI~\cite{CXL,openCAPI,genz,CCIX,benton2017ccix,ramdas2021enzian} to integrate local and remote memory within the same processor system.
\BLUE{However, HMD  systems come with a cost of higher access latency over an interconnect fabric that leads to  access cost of 100-1000x compared to NUMA systems leading 3-6x performance degradation}

a significant challenge arises when accessing remote memory over an interconnect fabric: increased memory access latency that can lead to severe application performance degradation~\cite{gouk2023memory,gouk2022direct,patke2022evaluating,pinto2020thymesisflow,lim2009disaggregated,syrivelis2017software}.
\BLUE{Increased memory access latency, as shown in Figure~\ref{fig:intro_degradation}, can lead to 3-6x worse performance degradation for datacenter applications in HMD systems compared to other tiered memory systems.}
Operating systems tackle this performance degradation by employing \emph{page migration}~\cite{linux_migration}, which promotes pages that are likely to be accessed from remote to local memory, thereby enhancing spatial locality and minimizing cross-node communication.
\\


\begin{figure}[ht]
    \includegraphics[width=3.3in]{resources/motivation/intro_degradation.pdf}
\vspace{1ex}
\caption{Increased network access cost leads to severe and variable performance degradation in HMD systems. Applications were run with the TPP page migration mechanism, now default in Linux~\cite{maruf2022tpp}. Variable network access latency is introduced using multi-application contention.}
\label{fig:intro_degradation}
\end{figure}

\noindent \textbf{Limitations of Existing Page Migration Mechanisms.}
While a myriad of page migration algorithms have been proposed for tiered memory systems~\cite{linux_migration,kim2021exploring,verghese1996operating,agarwal2017thermostat,yan2019nimble,ren2023hm,kannan2017heteroos,raybuck2021hemem,li2023hopp}, we identify two unique limitations that prevent them from achieving the best performance in HMD systems:
\begin{enumerate}[label=\textbf{L\arabic*}:,wide=0pt]
    \item \emph{Oblivious to Network\footnote{Any mention of network in this paper refers to the memory interconnect which is different from the regular datacenter network.} Transfer Cost and Contention.} The benefit of page migration is realized only when the improvement in access locality exceeds the page migration cost on the network.
    In previous tiered memory systems, network transfer was not the dominant cost (as we show in Section~\ref{ss:page_migration_characterization}), and not considering its effects was the correct design choice.
    However, ignoring the network transfer cost in HMD systems can lead to suboptimal decision-making, for example, due to excessive page migrations during periods of network contention.
    
    % inherently algorithms are noisy/inacccurate and are not able to capture access locality benefit leading to excessive migrations
    % Because of this excessive migration and high network cost in HMD, application performance degrades significantly
    % What is inacccurate about current algorithms?
    %They all estimate future memory access patterns using a moving average, which is a poor measure
    % As application patterns get more dynamic, (magnitude of gradient of access rate with time) you should give less weightage to past (smaller window)
    % smaller window is what we capture with burst duration
    \item \emph{Reliance on Inaccurate Page Access Estimation.} Page migration inherently requires the estimation of memory access patterns to decide which pages should be migrated to minimize memory access latency.
    This estimation consists of both the page access counts and the temporal context (time interval) during which the access counts are relevant. 
    Previously proposed mechanisms typically use moving averages~\cite{raybuck2021hemem,memtis_sosp} or bit vectors~\cite{kwon2016coordinated} that, when used in isolation, may not be accurate estimators of access patterns, especially when the access patterns are dynamic.
    Even with ML-based prediction of page access patterns~\cite{shumway2017arima,yu2019review}, we show that it is insufficient and costly for online page migration decision problems.
\end{enumerate}


\noindent \textbf{\sysname Design.}
To resolve the limitations of previous page migration mechanisms in the context of HMD systems, we introduce \sysname.
\sysname consists of two major components: \emph{Page Telemetry} and \emph{Page Promoter}.

Addressing \textbf{L2}, \emph{Page Telemetry} improves the accuracy of page access estimation by differentiating between stationary and dynamic application access patterns.
Differentiation between the two patterns is enabled by calculating the size of each \textit{interval} (i.e., ``burst duration'') in which the access pattern does not vary significantly.
Smaller burst durations imply that the application memory access pattern is dynamic (and vice versa for larger ones).
Page Telemetry coalesces similar access rates into the same interval, and the burst duration is calculated as the length of this interval.

Addressing \textbf{L1}, \emph{Page Promoter} adopts a network-aware page migration policy that considers the trade-off between the cost of page transfer and memory access locality benefit (we develop an analytical model to consider this trade-off in Section~\ref{ss:network_cost_model}) within the constraint of limited local memory allocation.
The input to the Page Promoter includes measurements from Page Telemetry, application memory allocation, and network telemetry.
The page promotion decision is based on a contextual multi-armed bandits agent that is trained using historical application runtime data.
We also provide an alternate heuristic-based network adaptive policy if no application training data is available\footnote{The heuristic-based approach is only network adaptive but not adaptive to the dynamicity of application access patterns}.

\sysname consists of both a kernel and a userspace component. Page Telemetry and Page Promoter are implemented in the \texttt{Linux kernel v5.8.0} in less than 700 modified LOC.
The contextual multi-armed bandits agent is implemented as a userspace daemon to minimize the overhead of switching execution to the kernel space.
Upon acceptance, we will open-source the implementation of \sysname.

\noindent \textbf{Results.}
We evaluated \sysname with common cloud applications, including in-memory databases~\cite{stonebraker2013voltdb}, in-memory key-value stores~\cite{carlson2013redis}, ML inference~\cite{vaswani2017attention}, graph analytics kernels~\cite{murphy2010introducing}, and scientific computational code~\cite{gahvari2011modeling} on a real disaggregated memory prototype, ThymesisFlow~\cite{thymesisflow}. We also compared INDIGO with state-of-the-art page migration techniques and recent research work available in the literature, such as TPP~\cite{maruf2022tpp}, Nimble~\cite{yan2019nimble}, and MEMTIS~\cite{memtis_sosp}.

%if workloads are repetitive, INDIGO makes the most sense to use (support with characterization numbers)
\begin{enumerate}[label=\arabic*.,wide=0pt]
    \item \emph{Improved Application Performance.} \sysname improves application performance by up to 50--70\% compared to other state-of-the-art page migration policies across low to high local-to-remote memory allocation ratios. The network adaptive policy also offers an improvement of up to 20--50\% in the presence of network contention.


    \item \emph{Unlocking Memory Offload.}
    For applications such as ML inference, \sysname can match full local memory execution performance with limited local memory allocation, thereby enabling 80--90\% offload of the application working set\footnote{The ``working set'' of an application is the collection of memory pages that are currently owned by the application.} from local to remote memory.
    % Such offloading can enable inference on large models such as GPT-3~\cite{floridi2020gpt} that will not fit in a single-node system.

    \item  \emph{Reduced Network Traffic.} \sysname reduces network traffic by up to 3\texttimes{} compared to other policies, such as MEMTIS, TPP, and Nimble, while improving the overall application performance. 
    The decreased network traffic leads to reduced contention and improved colocation for multiple applications that share the network. 

    \item \emph{Minimal Training Costs.} We trained \sysname with context caching that reduced training time by 100\texttimes{} to $\sim$1000 runs, thereby also reducing the cost of retraining. 
    Our evaluation also shows that \sysname, when exclusively trained on a particular application, will perform equally well on other, similar applications without any retraining.
    For example, there is a $<$5\% drop in application performance when one trains \sysname on a breadth-first search (BFS) application but tests the trained model on a single source shortest path (SSSP) application (with no retraining/adaptation).
\end{enumerate} 


\noindent \textbf{Putting \sysname in perspective.}
The problem of deciding the location of memory pages is also present in other OS-based approaches to memory disaggregation that use RDMA along with a swap cache such as InfiniSwap~\cite{gu2017efficient}, Leap~\cite{al2020effectively},
Fastswap~\cite{amaro2020can},
and Hermit~\cite{qiao2023hermit}.
However, these RDMA-based systems are fundamentally different from HMD systems, as they emulate disaggregated memory via the kernel; rather than extending the address space.
Consequently, \emph{they do not have the option of keeping the accessed page in remote memory};  it has to be brought to local memory.
That changes the decision problem, and the analytical model (later presented in Section~\ref{ss:network_cost_model}) no longer holds. 
The page-to-transfer decision becomes a prefetching problem as opposed to a migration problem.

Page migration in HMD systems is also unique compared to data placement in tiered storage systems, as network latency and bandwidth~\cite{li2023pond} are typically not the bottleneck factors in accessing slower storage devices~\cite{xu2015performance}.

